Can poachers find animals from public camera trap images?

To protect the location of camera trap data containing sensitive, high-target species, many ecologists randomly obfuscate the latitude and longitude of the camera when publishing their data. For example, they may publish a random location within a 1km radius of the true camera location for each camera in their network. In this paper, we investigate the robustness of geo-obfuscation for maintaining camera trap location privacy, and show via a case study that a few simple, intuitive heuristics and publicly available satellite rasters can be used to reduce the area likely to contain the camera by 87% (assuming random obfuscation within 1km), demonstrating that geo-obfuscation may be less effective than previously believed.

==> authors.tex <==
Sara Beery*$^\dagger$, Elizabeth Bondi*$^\ddag$\\
\begin{tabular}{ccc}
California Institute of Technology$^\dagger$ & Harvard University$^\ddag$ \\


\end{tabular} \\
*Equal contribution
